IDRBench: Understanding the Capability of Large Language Models on Interdisciplinary Research

Innovation is a key driving force of human civilization. As the body of knowledge has grown considerably, bridging knowledge across different disciplines, where significant innovation often emerges, has become increasingly challenging. The recent advancements in machine learning models, particularly Large Language Models (LLMs), have provided effective access to extensive knowledge sources and shown impressive abilities in reasoning, rendering significant opportunities for interdisciplinary discovery. Our research aims to understand the capabilities of state-of-the-art LLMs in integrating knowledge from different fields for interdisciplinary research (IDR). To address this fundamental problem, we introduce IDRBench, a pioneering framework that includes both datasets and evaluation tasks: (1) IDR Paper Identification, (2) IDR Idea Integration, and (3) IDR Idea Recommendation. Our study on ten mainstream LLMs provides a comprehensive analysis of their behavior and establishes benchmarks and baselines for future research. To the best of our knowledge, IDRBench is the first to provide a comprehensive investigation of LLMs' IDR capability.

==> Texts/s1_intro_old.tex <==
% S1
\section{Introduction}
\label{sec:introduction}

%\begin{displayquote}
%\textit{``If you would understand anything, observe its beginning and its development.''}
%\par\hfill---\textit{Aristotle}
%\end{displayquote}

Aristotle, one of history's greatest polymaths, made enduring integrations across philosophy, biology, physics, logic, and more areas, shaping centuries of intellectual development. However, as the body of scientific knowledge has grown considerably, modern science has fragmented into ever more specialized fields, making it increasingly difficult to bridge interdisciplinary scientific domains. At the same time, recent advancements in Large Language Models (LLMs) \cite{gpt_4, openai_o1_2024, llama, claude, deepseek}, with improved reasoning abilities and access to massive corpora spanning diverse scientific fields, have shown enormous potential in scientific discovery, supporting promising new approaches to \textbf{interdisciplinary research}. 
Indeed, frameworks that endow LLMs with nascent abilities to conduct research ideation \cite{Contents_Context_2021, FullyAutomatedSciDiscovery_2024}, deploy research codes \cite{research_coding}, or even compose detailed research proposals \cite{Stanford_Novelty_2024} have catalyzed the emergence of a handful of benchmarks measuring LLM's ideation quality \cite{IdeaBench_2024, SchNovel_2024, research_bench, yang2025moosechem}, marking a promising new paradigm of LLM-accelerated scientific research. 

While these frameworks and benchmarks provide solid evaluations on the outcome quality of the proposed ideas in generic research or single-disciplines, there is a notable gap in evaluating LLM's ability to perform ideation under the context of \textit{Interdisciplinary Research (IDR)}. According to the widely accepted definition ~\cite{HowToMeasureIDR_2024,ConvergenceIDR_2015,UncertaintyIDR_2023,MultiInterTrans_IDR_2022}, Interdisciplinary Research is \textit{``a mode of research ... that \textbf{integrates} information, data, techniques, tools, perspectives, concepts, and/or theories from two or more disciplines or bodies of specialized knowledge to advance fundamental understanding or to solve problems whose solutions are beyond the scope of a single discipline or area of research practice.''}. 


%\daniel{Widely used~\cite{HowToMeasureIDR_2024,ConvergenceIDR_2015,UncertaintyIDR_2023,MultiInterTrans_IDR_2022}, the definition of Interdisciplinary Research is : \textit{``A mode of research ... that \textbf{integrates} information, data, techniques, tools, perspectives, concepts, and/or theories from two or more disciplines or bodies of specialized knowledge to advance fundamental understanding or to solve problems whose solutions are beyond the scope of a single discipline or area of research practice.''}. }

\daniel{Existing works that explicitly explore the potential of using LLMs to tackle IDR problems \cite{IDRClassification_2024,IdentifyingIDRProblema_2024, Personaflow_2024, Disciplink_2024} often conduct investigations that provide novel different approaches and frameworks. However, none of them devote attention to thoroughly evaluate the inherent LLM capability of performing IDR tasks. As a result, the excessive focus on outcome-driven analyses of LLMs tends to overlook IDR's core characteristic of \textbf{integration of knowledge across distinct disciplines}, leaving scarce evidence to answer this key research question: \textbf{\textit{Are LLMs inherently capable of integrating different disciplines and provide clear descriptions for interdisciplinary research?}} }

Answering this question is not easy, since we need to evaluate whether an LLM can capture the task of the ``Eureka'' moment in interdisciplinary research, connecting knowledge from different disciplines to make a new scientific discovery~\cite{eureka}. To the best of our knowledge, none of the existing works have evaluated such capability of the state-of-the-art LLMs. One major issue that hinders such evaluation is the lack of a dedicated benchmark specifically designed for interdisciplinary research. The absence of an benchmark also makes it more difficult to measure the actual improvements brought by new approaches when they are compared to the baselines, increasing the risk of misleading comparisons and reducing the reproducibility of IDR findings. 



\begin{figure}
  %\vspace*{-7mm}
  \begin{center}
    \includegraphics[width=0.8\linewidth]{Figures/data_structure.png}
  \end{center}
  \caption{Triplet data format in IDRBench - Showing that Papers $P_B$ and $P_C$ are integrated (more than merely referenced) to generate the IDR Paper $P_A$. To obtain a positive triplet, the annotators need to identify $P_A$ from the candidate pool, then figure out the key cited papers $P_B$ and $P_C$ that play central roles in deriving the IDR idea.}  
  \label{fig: data_struct}
  \vspace*{-6mm}
\end{figure}
%\begin{wrapfigure}{r}{0.37\textwidth}
%  \vspace*{-7mm}
%  \begin{center}
%    \includegraphics[width=0.9\linewidth]{Figures/data_structure.png}
%  \end{center}
%  \caption{Triplet data format in IDRBench - Showing that Papers $P_B$ and $P_C$ are integrated (more than merely referenced) to generate the IDR Paper $P_A$. To obtain a positive triplet, the annotators need to identify $P_A$ from the candidate pool, then figure out the key cited papers $P_B$ and $P_C$ that play central roles in deriving the IDR idea.}  
%  \label{fig: data_struct}
%  \vspace*{-6mm}
%\end{wrapfigure}

 \daniel{Therefore, to contribute to understanding LLMs' abilities in IDR as a closed-book -- without considering any specific framework to enhance LLM -- we took an important step to introduce \textbf{IDRBench}, a pioneering benchmark designed for IDR assessment. IDRBench adopts the perspective of a progressive assessment of LLMs conducting interdisciplinary research by introducing three tasks, including: \textit{(i) IDR Paper Identification (IPI)}, evaluating LLM's ability to classify interdisciplinary papers; \textit{(ii) IDR Idea Integration (I3)}, testing LLM's ability to combine papers from distinct disciplines into feasible and novel IDR; and \textit{(iii) IDR Idea Recommendation (I2R)}, evaluating LLM's ability to recommend the most appropriate IDR paper given a list of unrelated papers. Tasks I3 and I2R focus more on the LLM’s integration capability, whereas task IPI represents a typical step when identifying whether a paper is an IDR or not. 
 
  
From IDR definition, we understand that the spectrum between non-IDR and IDR papers contains many nuances, and it is not always easy to determine whether a paper is interdisciplinary. However, we argue that within this spectrum, one can focus on its more clear-cut (or extreme) regions, specifically in order to define a paper as an IDR or on the scope on tangible/objective integration of IDR ideas based on citations papers. Therefore, the proposed tasks help us to frame the IDR challenge in an accessible way, assessing the ability of LLMs to automatically -— without human interference -— integrate different disciplines when generating novel IDR. Moreover, these tasks are grounded in real scenarios that human researchers typically encounter in interdisciplinary work, a point also supported in the IDR's literature \cite{MultiInterTrans_IDR_2022}.}
 
%--, that considering the same model's release used in our work, can be applied for future researchers without leakage issues

Thus, to gauge LLMs' performance on these tasks, the IDRBench dataset is structured as a knowledge triplet as illustrated in Figure \ref{fig: data_struct}. For instance, an IDR paper titled ``Tumor Location-weighted Contrastive Learning:  Improving the Explainability of Pediatric Brain Tumor Diagnosis'' serves as ``Citing Paper $P_A$'', accompanied by two ``Cited Papers'' $P_B$ and $P_C$ from the disciplines of quantitative biology and computer science, respectively. In this way, an IDR triplet is represented in the form $[P_A; (P_B, P_C)]$ and it can be generalized to include more than two cited papers. \footnote{ \daniel{Although our triplet representation can be described with many cited papers, in Section 3 we show that 93\% of IDR papers associated with more than one discipline are described by the authors as a combination of only two primary cited papers.}}


\daniel{One important issue in this triplet-based evaluation of LLMs is whether the model’s training data already contains knowledge of the existence of the ``Citing Paper $P_A$'' and its references to the `Cited Papers'' $P_B$ and $P_C$. Such data leakage could naturally influence the LLM’s decisions regarding IDR behavior. To mitigate this issue, we crawled the most recent papers from the ArXiv dataset that have not yet been published in any venue, ensuring that each paper $P_A$  was uploaded after the LLM’s release and therefore could not have been included in its training data.

Using ArXiv as a reliable dataset, we provide a comprehensive evaluation on 10 mainstream LLMs, establishing the first quantified baseline that measures the inherent capability of various LLMs in integrating IDR. We observe that  LLMs demonstrate an advantage over both IDR Idea Integration (I3) and IDR Idea Recommendation (I2R) tasks, while leaving room for improvement in the IDR Paper Identification (IPI) task.
Further analysis on these results reveals that although LLMs have developed some awareness of the IDR notions in IDR classification and recommendation, they are still struggling to yield quality IDR ideas in a plug-and-play fashion under real-world settings, leaving space for future improvements. }


\henry{Answering this question is not easy, as the design of such benchmark needs to overcome two major obstacles: (1) the fact that the spectrum between non-IDR and IDR papers contains many nuances, meaning that it is not always easy to determine whether a paper is interdisciplinary, and (2) the suit of tasks within the benchmark should be capable of evaluating whether an LLM can capture the task of the ``Eureka'' moment in IDR, connecting knowledge from different disciplines to make a new scientific discovery~\cite{eureka}. }

\henry{To overcome the first challenge, we take the observation from \cite{citations_equal} that the major innovation of a given paper is often derived from a leading idea within a cluster of papers from its citation section. We hereby extend this notion and argue that one can differentiate an IDR paper that is on the more clear-cut (or extreme) regions of the spectrum based on the integration of key citation papers. Thus, to effectively represent citation-based IDR, we introduce a knowledge triplet illustrated in Figure \ref{fig: data_struct}. For instance, an IDR paper titled ``Tumor Location-weighted Contrastive Learning:  Improving the Explainability of Pediatric Brain Tumor Diagnosis'' serves as ``Citing Paper $P_A$'', accompanied by two ``Cited Papers'' $P_B$ and $P_C$ from the disciplines of quantitative biology and computer science, respectively. In this way, an IDR triplet is represented in the form $[P_A; (P_B, P_C)]$ and it can be generalized to include more than two cited papers. \footnote{Although our triplet representation can be described with many cited papers, in Section 3 we show that 93\% of IDR papers associated with more than one discipline are described by the authors as a combination of only two primary cited papers.}}

\henry{To address the second challenge, we introduce \textbf{IDRBench}, a novel evaluation framework that contains a progressive assessment of LLMs conducting interdisciplinary research in a closed book manner, without considering any specific framework to enhance LLMs' original ability. \textbf{IDRBench} includes three tasks, including: \textit{(i) IDR Paper Identification (IPI)}, evaluating LLM's ability to classify interdisciplinary papers; \textit{(ii) IDR Idea Integration (I3)}, testing LLM's ability to combine papers from distinct disciplines into feasible and novel IDR; and \textit{(iii) IDR Idea Recommendation (I2R)}, evaluating LLM's ability to recommend the most appropriate IDR paper given a list of unrelated papers. Tasks I3 and I2R focus more on the LLM’s integration capability, whereas task IPI represents a typical step when identifying whether a paper is an IDR or not.}

\henry{The dataset in \textbf{IDRBench} is derived from a subset containing the most recent papers from the ArXiv platform that have not yet been published in any venue and construct the paper triplet based on these data. Such choice of design is intended to enhance the efficacy of evaluation and avoid the data leakage issue, as it ensures that each paper $P_A$ was uploaded after the LLM’s release and therefore could not have been included in its training data. We then provide a comprehensive evaluation on 10 mainstream LLMs, establishing the first quantified baseline that measures the inherent capability of various LLMs in IDR tasks. We observe that \textbf{This part should also include results from human evaluation}}

% LLMs demonstrate an advantage over both IDR Idea Integration (I3) and IDR Idea Recommendation (I2R) tasks, while leaving room for improvement in the IDR Paper Identification (IPI) task. Further analysis on these results reveals that although LLMs have developed some awareness of the IDR notions in IDR classification and recommendation, they are still struggling to yield quality IDR ideas in a plug-and-play fashion under real-world settings, leaving space for future improvements. 




%It is worth to remark, that although there is consensus on the significance of facilitating IDR, no off-the-shelf protocol is defined rigorously on the specific process of conducting IDR with LLM methods. 

 
We summarize our main contributions as follows: 
\begin{itemize}[leftmargin=0.4cm, itemsep=0em] 
    \item We release IDRBench, the first benchmark to comprehensively evaluate LLMs' abilities as closed-book settings in Interdisciplinary Research (IDR), including a human-annotated dataset and a suite of three dedicated tasks: IDR Paper Identification (IPI), IDR Idea Integration (I3), and IDR Idea Recommendation (I2R), enabling a comprehensive assessment of LLM's IDR ability.
    \item Our evaluation and analysis results reveal divergent performance across LLMs, showcasing their advantages in both the I3 and I2R tasks, while leaving notable room for improvement in the IPI task. Further analysis also suggests that LLMs are still struggling to provide high-quality IDR proposals despite showing early signs of IDR awareness.       
    \item We establish a standardized framework for extracting IDR data efficiently, minimizing human annotation effort while ensuring consistent and reliable evaluation. 
\end{itemize}


==> Texts/s1_intro_old_2601280449.tex <==
% S1\
\vspace{2mm}
\section{Introduction} %\textcolor{red}{This introduction section could be a bit concise?}
\label{sec:introduction}

% \daniel{Maybe we can find same quote that consider the Aristotle's ideas integration .. }
\begin{displayquote}
\textit{``If you would understand anything, observe its beginning and its development.''}
\vspace{-2mm}
\par\hfill---\textit{Aristotle}
\end{displayquote}
\vspace{-2mm}
Aristotle, one of history's greatest polymaths, made enduring contributions across philosophy, biology, physics, logic, and more areas, shaping centuries of intellectual development. However, as the body of knowledge has grown considerably, modern fields of studies have fragmented into ever more specialized areas, making it increasingly difficult for humans to digest and integrate knowledge from different domains for  interdisciplinary research (IDR). 
On the other hand, recent advancements in Large Language Models (LLMs) \cite{gpt_4, openai_o1_2024, llama, claude, deepseek} have provided significant potentials in scientific discovery due to the knowledge they store and the increasing ability in reasoning, which have begun to show capabilities ranging from research ideation \cite{Contents_Context_2021, FullyAutomatedSciDiscovery_2024} 
%and composing detailed research proposals \cite{Stanford_Novelty_2024} 
to deploying research codes \cite{research_coding}, including research that catalyzed the emergence of novel evaluations that attempted to understand LLMs' novelty \cite{IdeaBench_2024, SchNovel_2024, research_bench, yang2025moosechem}, marking a promising new paradigm of LLM-accelerated scientific research.


%While these frameworks and benchmarks provide solid evaluations on the outcome quality of the proposed ideas in generic research or single-disciplines, 
However, there is a notable gap in studying the state-of-the-art of LLMs ability in  \textit{Interdisciplinary Research (IDR)}, as IDR has become increasingly challenging.  
The absence of a dedicated benchmark that assesses LLMs on integrating knowledge across distinct disciplines leaves scarce evidence to answer this key research question: \textbf{\textit{Are LLMs capable of conducting interdisciplinary research?}}


Specifically, we asssess the state of the art of LLMs in connecting knowledge from different disciplines to perform interdisciplinary research. To address this fundamental problem, we introduce IDRBench, a pioneering framework that include both datasets and  tasks designed to assess LLMs' basic interdisciplinary research abilities.



%Also, the excessive focus on outcome-driven analyses overlooks the core characteristics within the widely accepted definition of IDR ~\cite{HowToMeasureIDR_2024,NRC2014Convergence, UncertaintyIDR_2023,MultiInterTrans_IDR_2022} to \textit{``\textbf{integrate} information, data, techniques, tools, perspectives, concepts, and/or theories from two or more disciplines or bodies of specialized knowledge to advance fundamental understanding or to solve problems whose solutions are beyond the scope of a single discipline or area of research practice.'' } Moreover, existing works that explore the potential of using LLMs to tackle IDR problems \cite{IDRClassification_2024,IdentifyingIDRProblema_2024, Personaflow_2024, Disciplink_2024} often emphasize on either proposing novel frameworks and approaches, or merely offering limited qualitative comparisons, yet lacking a thorough investigation into LLMs' inherent IDR capability. 



Answering this question is not easy, as the design of such a benchmark needs to overcome two major obstacles: (1) the spectrum between non-IDR and IDR papers contains many nuances, meaning that it is not always easy to determine whether a paper is interdisciplinary or not, and (2) the suit of tasks within the benchmark should be capable of evaluating whether an LLM can capture the ``Eureka'' moment in IDR, connecting different disciplines to make a new scientific discovery~\cite{eureka}. 


%To address the second challenge, we introduce \textbf{IDRBench}, a novel evaluation benchmark that contains a progressive assessment of LLMs conducting IDR in a closed book manner, without considering any specific framework to enhance LLMs' original ability. 

%The dataset in IDRBench is derived from a subset containing the most recent papers from the ArXiv Platform\footnote{https://arxiv.org/} that have not yet been published in any venue. Thus we intend to avoid potential data leakage, as each paper $P_A$ was \textbf{uploaded after} the LLM’s release and therefore could not have been included in its training data. IDRBench includes three tasks: \textit{(i) IDR Paper Identification (IPI)}, evaluating LLM's ability to classify IDR papers; \textit{(ii) IDR Idea Integration (I3)}, testing LLM's ability to combine papers from distinct disciplines into feasible and novel IDR; and \textit{(iii) IDR Idea Recommendation (I2R)}, evaluating LLM's ability to recommend the most appropriate IDR paper given a list of unrelated papers. Tasks I3 and I2R focus more on the LLM’s integration capability, whereas task IPI focus on identifying whether a paper is an IDR or not.




In order to answer our research question, we perform a comprehensive evaluation of 10 mainstream LLMs, establishing the first quantified baseline for IDR related tasks. Our results reveal that while \textbf{LLMs exhibit promising integration capabilities (Macro-F1 score of 0.822 ), their understanding of what truly constitutes interdisciplinary remains limited (an average Macro-F1 of only 0.353).} Moreover, we observe a clear trade-off in model behavior: some models tend to over-generate interdisciplinary claims, leading to excessive false positives, while others are overly conservative, producing high false-negative rates. We summarize our key contributions: 

%Specifically, the best-performing model achieves a Macro-F1 score of 0.822 on valid IDR integration, a finding further corroborated by human evaluations. However, when distinguishing true IDR integrations from feasible but non-IDR alternatives, models struggle substantially, attaining an average Macro-F1 of only 0.353, indicating limited IDR awareness rather than a lack of generative capacity.


%We perform a comprehensive evaluation of 10 mainstream LLMs to establish the first quantified baseline for IDR related tasks. 
% current version:
% Our results reveals that LLM already possess promising capabilities in making valid idea integrations, with the best performing model achieving 0.822 Macro-F1 score in one of our sub integration tasks. However, we also notice that models still struggle to foster sufficient IDR awareness, achieving an average Macro-F1 score of 0.353 when selecting correct IDR integrations from feasible but non-IDR negatives. These results highlights both the strengths and shortcomings of existing state-of-the-art models, which facilitates our understanding of LLM's boundary when handling tasks under the IDR context. 
% updated version
%Our results reveals promising capabilities for models to make valid integrations in IDR, with the best performing model achieving 0.822 Macro-F1 score, which is further corroborated by human evaluations on IDR idea quality ratings. However, these models still struggle to foster sufficient IDR awareness, achieving an average Macro-F1 score of 0.353 when selecting correct IDR integrations from feasible but non-IDR negatives. We summarize our key contributions: 


\vspace{-3mm}
\begin{enumerate}[leftmargin=10pt, itemsep=0pt]

    \item \textbf{IDRBench}, we introduce the first comprehensive, closed-book benchmark designed to evaluate LLMs on interdisciplinary integration. The suite includes a high-quality human-annotated dataset across multiple specialized IDR tasks;
    %version 1
    %IDRBench is the first benchmark to comprehensively evaluate LLMs' abilities in a closed-book manner using a human-annotated dataset and a suite of IDR tasks.
    
    %Vestion 0
    % \item Our main results show that models perform better in identifying IDR feasibility rather than maintaining IDR awareness. 
    \item \textbf{Behavioral Divergence and Reasoning Trade-off}, error analysis show that models are divided in either providing excessive false positives or false negatives in idea integration, along with reasoning models being inferior than non-reasoning models\footnote{This finding is corroborated by prior studies~\cite{luyten2026reasoningcreativitytradeoffcreativitydrivenproblem, mohammadi2024creativityleftchatprice} that examine generative creativity within the optimization process.}.
    
    %vesion: 0
    % into either being optimistic in providing false positive integrations or being conservative in providing false negative integrations. Also interestingly, non-reasoning models are more balanced between IDR feasibility and awareness than reasoning models
     
         
    \item \textbf{An efficient and scalable data collection pipeline}, accompanied by preliminary explorations of downstream applications, demonstrating how IDRBench can support broader research on interdisciplinary discovery and evaluation.
    
    %Version1: We provide an efficient and scalable data collection pipeline with some preliminary explorations on use cases that extends the utility of IDRBench.

    %Version0
    %We develop a data collection pipeline based on our paper triplet structure, focusing on efficient and sustainable IDR data extraction while minimizing human annotation effort. This pipeline also ensures consistent and reliable evaluation as well as promoting future up-scaling based on our annotated dataset.
    % that promotes sustainability for extracting IDR data efficiently, minimizing human annotation effort while ensuring consistent and reliable evaluation. 
\end{enumerate}


\vspace{-3mm}


% Daniel's comments below
% -------------------------------------------------------------------

% \daniel{A comprehensive evaluation of 10 mainstream LLMs establishes the first quantified baseline for IDR tasks, yielding several key insights: First, we observe that while some models are optimistically inclined to identify and suggest IDR ideas, others remain conservative. Second, while the models are capable of assessing the feasibility of IDR integration, they are less effective at maintaining awareness of the IDR definition. Third, non-reasoning models achieve a better balance between TPR and TNR than reasoning models. Complementing the evaluation, we provide a comprehensive data collection pipeline that enables future work to generate positive and negative IDR instances.}


%  %We develop a data collection pipeline based on our paper triplet structure, focusing on efficient and sustainable IDR data extraction while minimizing human annotation effort. This pipeline also ensures consistent and reliable evaluation as well as promoting future up-scaling based on our annotated dataset
% % \textbf{This part should also include results from human evaluation}

% % LLMs demonstrate an advantage over both IDR Idea Integration (I3) and IDR Idea Recommendation (I2R) tasks, while leaving room for improvement in the IDR Paper Identification (IPI) task. Further analysis on these results reveals that although LLMs have developed some awareness of the IDR notions in IDR classification and recommendation, they are still struggling to yield quality IDR ideas in a plug-and-play fashion under real-world settings, leaving space for future improvements. 


% %It is worth to remark, that although there is consensus on the significance of facilitating IDR, no off-the-shelf protocol is defined rigorously on the specific process of conducting IDR with LLM methods. 

 
% We summarize our main contributions as follows: 
% \begin{itemize}[leftmargin=0.4cm, itemsep=0em] 
%     \item We release IDRBench, the first benchmark to comprehensively evaluate LLMs' abilities as closed-book settings in Interdisciplinary Research (IDR), including a human-annotated dataset and a suite of three dedicated tasks.
%     % : IDR Paper Identification (IPI), IDR Idea Integration (I3), and IDR Idea Recommendation (I2R), enabling a comprehensive assessment of LLM's IDR ability.
%     \item Our evaluation together with human evaluation results reveal divergent performance across LLMs, also indicating the promising development of these models to assist human experts in providing useful and correct IDR ideas. %Further analysis also suggests that LLMs are still struggling to provide high-quality IDR proposals despite showing early signs of IDR awareness.       
%     \item 
    
    
%     %We develop a data collection pipeline based on our paper triplet structure, focusing on efficient and sustainable IDR data extraction while minimizing human annotation effort. This pipeline also ensures consistent and reliable evaluation as well as promoting future up-scaling based on our annotated dataset.
    
    
%     % that promotes sustainability for extracting IDR data efficiently, minimizing human annotation effort while ensuring consistent and reliable evaluation. 
% \end{itemize}


% -------------------------------------------------------------------

